STRODE: Stochastic Boundary Ordinary Differential Equation

Perception of time from sequentially acquired sensory inputs is rooted in everyday behaviors of individual organisms. Yet, most algorithms for time-series modeling fail to learn dynamics of random event timings directly from visual or audio inputs, requiring timing annotations during training that are usually unavailable for real-world applications. For instance, neuroscience perspectives on postdiction imply that there exist variable temporal ranges within which the incoming sensory inputs can affect the earlier perception, but such temporal ranges are mostly unannotated for real applications such as automatic speech recognition (ASR). In this paper, we present a probabilistic ordinary differential equation (ODE), called STochastic boundaRy ODE (STRODE), that learns both the timings and the dynamics of time series data without requiring any timing annotations during training. STRODE allows the usage of differential equations to sample from the posterior point processes, efficiently and analytically. We further provide theoretical guarantees on the learning of STRODE. Our empirical results show that our approach successfully infers event timings of time series data. Our method achieves competitive or superior performances compared to existing state-of-the-art methods for both synthetic and real-world datasets.

==> Table/2021_tbl_video_acc.tex <==
\begin{table}[htb!]
\vspace{-2mm} % 因为有hawks和exponential 俩个数据集，可能最好分开俩个表格（一个MSE 一个CD）
	\caption{ CS (mean$\pm$ std) and MSE Results on two subsets of Rotating MNIST Thumbnail}
	\label{tbl-video-acc}
	\centering
	\begin{tabular}{lcc}
		\toprule
		
		{\sf Model}  & CS  & MSE ($\times10^{-3}$)  \\ 
		\midrule
		NODE \cite{shi2015convolutional}                                  & 40.16 &11 \\
		ODE-RNN \cite{rubanova2019latent}                                & 41.87  &11            \\ 
		STRODE (Ours)                              & 43.13        &11      \\ 
		STRODE-RNN (Ours)                              & \textbf{46.56}        &11     \\ 
		\bottomrule
	\end{tabular}

\vspace{-3mm}
\end{table}











==> Table/tbl-SWB-30k.tex <==
\begin{table}[t]
\vspace{-2mm}
	\caption{WER (\%) on eval2000. }
	\label{tbl-SWB-30k}
	\centering
	\begin{tabular}{ll}
		\toprule
		
		{\sf Model}  & WER  \\ 
		\midrule
		Kaldi DNN \cite{kaldi}                                  & 26.8 \\
		SRU \cite{lei2017simple}                                   & 22.8              \\ 
		VSRU \cite{chung2015recurrent}                             & 22.6              \\ 
		RTN (Ours)                              & \textbf{20.8}             \\ 
		\bottomrule
	\end{tabular}
\vspace{-3mm}
\end{table}











==> Table/tbl-SWB-Q.tex <==
\begin{table}
%    \vskip -0.00in
	\caption{ Error rate(\%) of relation prediction on test set of RelationalSWB. }
	\label{tbl-SWB-Q}
	\centering
	\begin{tabular}{lll}
		\toprule
		
		{\sf Graph Type}  &  Err  \\ 
		\midrule
		Random Graph                           &50.0 \\
		Summary Graph                           & 28.6 \\
		Task-specific Graph                        & 28.7              \\ 

		\bottomrule
	\end{tabular}
	%\vskip -0.10in
\end{table}

==> Table/tbl-chime2.tex <==
\begin{table}
	\caption{WER (\%) on test set of CHiME-2. }
	\label{tbl-chime2}
	\centering
	\begin{tabular}{ll}
		\toprule
		
		{\sf Model}  & WER  \\ 
		\midrule
		Kaldi DNN \cite{kaldi} & 29.1 \\
		LSTM      \cite{huang2019recurrent} & 26.1                  \\ 
		SRU       \cite{huang2019recurrent} & 26.2                  \\ 
		RPPU      \cite{huang2019recurrent} & 24.4              \\ 
		\midrule
		Our SRU \cite{lei2017simple}  & 25.8                  \\ 
		VSRU \cite{chung2015recurrent}  & 25.8                  \\ 
		RRN \cite{palm2018recurrent}  & 24.8                  \\ 
		RTN (Ours)  & \textbf{23.9}                  \\ 
		\bottomrule
	\end{tabular}
	\vskip -0.1in
\end{table}











==> Table/tbl-chime2_time.tex <==
\begin{table}
  \caption{Model configuraions for all datasets and the training time for CHiME-2. L: number of layers; N: number of hidden states per layer;   P: number of model parameters; T: Training time per epoch (hr).}
\label{tbl-chime2_time}
%\vskip -0.1in
\begin{footnotesize}
  \centering
  \begin{tabular}{lcccc}
    \toprule
{\sf Model}  & {\sf L} & {\sf N} & {\sf P} & {\sf T} \\ 
    \midrule

SRU \cite{lei2017simple}                                     & 12            &1280            & 63M                                & 0.09                     \\ 
VSRU \cite{chung2015recurrent}                                     & 9            &1024            & 66M                                & 0.09                     \\ 

RRN \cite{palm2018recurrent}                                       & 9            &1024            & 64M                                & 0.09                     \\ 
RTN (Ours)                                     & 9            &1024            & 70M                                & 0.11                     \\ 
    \bottomrule
  \end{tabular}
  \end{footnotesize}
%  \vskip -0.2in
%   \vspace{5mm}
\end{table}









==> Table/tbl-chime5.tex <==
\begin{table} 
% \vspace{-6mm}
%\vskip 0.2cm
	\caption{WER (\%) on eval of CHiME-5. }
	\label{tbl-chime5}
	\centering
	\begin{tabular}{lll}
		\toprule
		
		{\sf Model}   &WER  \\ 
		\midrule
		%Kaldi GMM               & 64.8  \\
		Kaldi DNN \cite{kaldi}             & 64.5            \\ 
		SRU \cite{lei2017simple}                & 62.6            \\ 
		VSRU \cite{chung2015recurrent}         & 61.6            \\ 
		RTN (Ours)               & \textbf{57.4}           \\ 
		\bottomrule
	\end{tabular}
%	\vskip -0.4cm

\end{table}











==> Table/tbl-detail.tex <==
\begin{table*} [h]
%\begin{small}
  \caption{Detailed WER (\%) on the CHiME-2 test set.}
\label{tbl-detail}
  \centering
  \begin{tabular}{lllllll}

    \toprule

{\sf Model} & -6 dB & -3 dB & 0 dB & 3 dB & 6 dB & 9 dB \\
    \midrule
LSTM   \cite{huang2019recurrent}                      & 42.4  & 33.5  & 26.7 & 21.1 & 17.3 & 15.3 \\ 
SRU   \cite{huang2019recurrent}                       & 42.5  & 34.0  & 26.2 & 22.2 & 17.4 & 15.1 \\ 
RPPU     \cite{huang2019recurrent}                    & 39.9  & 31.1  & 24.9 & 20.3 & 16.0 & \textbf{13.2} \\ 
\midrule 

Our SRU \cite{lei2017simple}                          &42.1	&33	&26.1	&20.7	&16.8	&15.1 \\ 
VSRU      \cite{chung2015recurrent}                     &41.5	&32.8	&26.2	&20.9	&16.9	&16.1 \\ 
RRN \cite{palm2018recurrent}                          &40.2	&32.1	&25.9	&20.2	&16.2	&14.0 \\ 
RTN (Ours)                         & \textbf{39.0}  & \textbf{30.4}  & \textbf{25.4} & \textbf{19.4} & \textbf{15.5} & 13.8 \\ 
    \bottomrule
  \end{tabular}
  \vspace{0.3in} 
%\end{small}
\end{table*}

==> Table/tbl-models.tex <==
\begin{table}
	\caption{WER (\%) on evaluation sets of CHiME-2, WSJ0 and WSJ0\&1.}
	\label{tbl-models}
	\centering
	\begin{tabular}{llll}
		\toprule
		
		{\sf Model}  & CHiME-2 & WSJ0 & WSJ0\&1  \\ 
		\midrule
		LSTM       & 26.1                           & 2.8        & 7.4              \\ 
		SRU        & 26.2                           & 2.8        & 7.5              \\ 
		Quasi-RNN  & 26.1                           & 2.8        & 7.4              \\ 
		RPPU       & 24.4                           & 2.5        & 6.9             \\ 
		\bottomrule
	\end{tabular}
\end{table}











==> Table/tbl-similarity.tex <==
\begin{table}
\caption{Similarity with the ground-truth phoneme-level alignment for our baseline and  estimated alignment using RPP on development set of CHiME-2 }
\label{tbl-simi}
  \centering
  \begin{tabular}{lll}
    \toprule

Alignment type                 & Similarity(\%) \\
    \midrule
Baseline alignment    & 55.5           \\ 
Estimated alignment using RPP & \textbf{64.7}           \\ 
    \bottomrule
  \end{tabular}
\end{table}
